mmSnap: Bayesian One-Shot Fusion in a Self-Calibrated mmWave Radar Network

We present mmSnap, a collaborative RF sensing framework using multiple radar nodes, and demonstrate its feasibility and efficacy using commercially available mmWave MIMO radars. Collaborative fusion requires network calibration, or estimates of the relative poses (positions and orientations) of the sensors. We experimentally validate a self-calibration algorithm developed in our prior work, which estimates relative poses in closed form by least squares matching of target tracks within the common field of view (FoV). We then develop and demonstrate a Bayesian framework for one-shot fusion of measurements from multiple calibrated nodes, which yields instantaneous estimates of position and velocity vectors that match smoothed estimates from multi-frame tracking. Our experiments, conducted outdoors with two radar nodes tracking a moving human target, validate the core assumptions required to develop a broader set of capabilities for networked sensing with opportunistically deployed nodes.

==> ExperimentsAndDiscussion.tex <==
\section{Experimental Results}\label{sec:ExpAndResults}

\captionsetup[subfloat]{labelformat=simple}
\renewcommand{\thesubfigure}{(\alph{subfigure})}

\begin{figure*}[t!]
    \centering
    \subfloat[]{
        \includegraphics[width=0.24\textwidth]{X_R1_R2_Opt.pdf}%
        \label{b1}
    }
    \subfloat[]{
        \includegraphics[width=0.24\textwidth]{Y_R1_R2_Opt.pdf}%
        \label{b2}
    }
    \subfloat[]{
        \includegraphics[width=0.24\textwidth]{V_X_R1_R2_Opt.pdf}%
        \label{a1}
    }
    \subfloat[]{
        \includegraphics[width=0.24\textwidth]{V_Y_R1_R2_Opt.pdf}%
        \label{a2}
    }
    \vspace{-0.5em} % Adjust vertical space as needed
    \caption{$X, Y, V_X, V_Y$ estimates for Setup B2}
    \label{fig:one_shot_fusion}
\end{figure*}

\begin{figure}[t!]
    \centering
    \subfloat[]{\includegraphics[width=0.46\columnwidth]{ExpSetup1.png}\label{exp1}} 
    \vspace{0.5em}
    \subfloat[]{\includegraphics[width=0.46\columnwidth]{ExpSetup2.png}\label{exp2}}
    \caption{Experimental setups with two radar nodes.}
    \label{fig:exp_setups}
\end{figure} 

%\vspace{6em}
\begin{table}[t!]  % Change placement option
    \centering
    \renewcommand{\arraystretch}{1.3}
    \begin{tabular}{l c}
        \toprule
        \textbf{Parameter} & \textbf{Value} \\
        \midrule
        Carrier Frequency ($f_c$) & 76 GHz \\
        ADC Sampling Rate & 10 MHz \\
        Bandwidth & 4.24 GHz \\
        Chirp Slope & 83 MHz/s \\
        Frame Duration & 150 ms \\
        Number of Chirps per Frame & 180 \\
        Chirp Ramp Time & 60 s \\
        Range Resolution & 3.53 cm \\
        Doppler Resolution & 0.1827 m/s \\
        Max Unambiguous Range & 18.0723 m \\
        \bottomrule
    \end{tabular}
    \caption{Chirp Parameters for mmSnap Experiments}
    \label{tab:chirp_parameters}
\end{table}

In this section, we present experimental results for an outdoor two-radar node-based distributed network, used to track a single moving target following two distinct trajectories: (i) a straight line and (ii) random movement. The radar configurations and target trajectories are diagrammatically shown in Fig.~\ref{ExpSettings}. Three radar node configurations, labeled A–C, are investigated. In Configuration A, the two radar nodes are positioned facing each other. In Configuration B, the radar nodes are placed at a $90^\circ$ angle relative to each other. In Configuration C, the radar nodes are oriented in the same direction. In all configurations, the orientation of the radar nodes is indicated by the direction of the arrows, while the two distinct target trajectories are represented by the green curve. The experimental setup for radar node configuration C is depicted in Fig.~\ref{fig:exp_setups}. The radar nodes used for the experiments are TI AWR2243 mmWave MIMO radar boards operating at a carrier frequency of $76$ GHz with a bandwidth of $4.98$ GHz. The chirp parameters used for our experiments are detailed in Table~\ref{tab:chirp_parameters}. 

\subsection{Results and Discussion}

\textbf{Self-Calibration:} Firstly, to self-calibrate the two-radar network, we collect $90$-second sequences of a single moving human target within the overlapping FoV of the two radars. Based on the radar frame duration ($150ms$), this results in $600$ frames, which is the trajectory length utilized in the self-calibration algorithm. 


\begin{comment}
The distributions of position and orientation errors for the two target trajectories (straight and random) for the three different configurations are shown in Fig.~\ref{fig:positionorientationerror}.The position error is defined as the Euclidean distance between the observed position and the ground truth. The orientation error is the difference between the observed orientation from the other radar and the actual ground truth orientation. ({\color{blue} Note: Will edit this part after getting new results. The older once have discrepancies with ground truth.})

\subsection{Performance Evaluation}
\textbf{Self-Calibration:} The performance of our self-calibration algorithm was evaluated for all three radar node configurations and target trajectories, as shown in Fig.~\ref{ExpSettings}, by collecting $90$-second sequences of a single moving human target within the overlapping FoV of the radars. In our setup, one of the two radar nodes is selected as the reference for calibration. The position and orientation errors for the two target trajectories are shown in Fig.~\ref{fig:positionorientationerror} {\color{blue} (Need more info on what config etc)}.The position error is defined as the Euclidean distance between the observed position and the ground truth. The orientation error is the difference between the observed orientation from the other radar and the actual ground truth orientation.
\end{comment}

The self-calibration algorithm's performance is evaluated by comparing the trajectory RMSE values for the different node configurations and target trajectories. The corresponding values are tabulated in Table~\ref{tab:residual}. We observe that the calibration quality does not depend on the configurations themselves, but rather on the moving target trajectories. For each configuration, the self-calibration result for the random trajectory is worse than that of the straight trajectory. This is expected because arbitrary changes in the target movement can impact the quality of the tracks from each perspective, thereby reducing self-calibration efficacy. Fig.{\color{blue} Add Figure with track overlay} visually demonstrates the self-calibration algorithm, where the tracks from two radar perspectives are overlaid on top of each other and matched in a least-squares sense.

%For performing self-calibration, we collected 90s-long sequences of single targets moving in the overlapping FoV of the two radars. As mentioned before, we select one radar to be the reference. Considering one radar as the reference, we have the distributions of position and orientation errors for the different target trajectories in Fig.~\ref{fig:positionorientationerror}, where \textit{position error} be defined as the Euclidean distance between the other radar's observed position and the ground truth, and \textit{orientation error} be defined as the difference between the other radar's observed orientation and the actual ground truth orientation.

\begin{comment}
The self-calibration algorithm's performance is evaluated by comparing the minimum residual ($J_{min}$) values for the different node configurations and target trajectories. The corresponding values are tabulated in Table~\ref{tab:residual}. It is observed that Configuration A yields the highest values of \( J_{min} \) for each trajectory, while Configuration C results in the lowest. This can be attributed to the fact that the calibration results improve when the target moves closer to the broadside of both radars, leading to higher quality detections.
Additionally, while the \( J_{min} \) values are higher for the random trajectory compared to the straight trajectory for configurations A and C, the opposite trend is observed for configuration B. This can possibly be explained by the fact that, for configuration B, a target following a straight trajectory simultaneously moves away from the broadside of both nodes, leading to noisier detections compared to the random trajectory.
\end{comment}

%The calibration performance is illustrated by Table~\ref{tab:residual} where the minimum residual $J_{min}$ is evaluated for different trajectories and setups. Configuration A has the worst values of $J_{min}$ per trajectory, while C has the best. This can be attributed to the fact that the calibration results get better if the target moves close to the broadside of both radars, leading to better quality detections. Also, one interesting observation here is that, although for configs A and C, $J_{min}$ is higher for the random trajectory than the straight trajectory, for B it is the opposite. This might be possible because in the straight trajectory, the target simultaneously moves away from the broadside of both radars, leading to noisier detections, as opposed to the random trajectory.

\begin{table}[t]
  \centering
  \renewcommand{\arraystretch}{1.3}

  % Wrap tabular in \resizebox
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}l S S c S S c S S@{}}
      \toprule
      & \multicolumn{1}{c}{$A$} & \phantom{abc}& \multicolumn{1}{c}{$B$} &
        \phantom{abc} & \multicolumn{1}{c}{$C$} \\
      \midrule
      Straight Trajectory & 0.5664 && 0.5657 && 0.1783 \\
      Random Trajectory & 0.7076 && 0.6331 && 0.4426 \\
      \bottomrule
    \end{tabular}
  }%

  \caption{Trajectory RMSE values for different self-calibration scenarios}
  \label{tab:residual}
\end{table}



\begin{figure}[t!]
    \centering
    \subfloat[]{
        \includegraphics[scale=0.4]{b1_exp_regions.png}%
        \label{b1_exp_uncertainty}
    }\\
    \subfloat[]{
        \includegraphics[width=0.24\textwidth]{High_uncertainty.pdf}%
        \label{region_1}
    }
    \subfloat[]{
        \includegraphics[width=0.24\textwidth]{Low_uncertainty.pdf}%
        \label{region_2}
    }
    \vspace{-0.5em} % Adjust vertical space as needed
    \caption{Uncertainties in the two regions 1 and 2 for setup B1, visually represented by the velocity posterior distributions in b) and c), respectively}
    \label{fig:uncertainty}
\end{figure}

\textbf{One-Shot Fusion:} Once the radar network is self-calibrated, the Bayesian one-shot fusion estimates are derived using iid Gaussian priors for the position and velocity components, as shown in equation (\ref{Prior Distributions}). Although each radar can obtain range and angle measurements for the target, it can only measure the radial Doppler from the target motion. Therefore, as velocity estimates exhibit higher uncertainty than position, we set $\sigma_x = \sigma_y = 1m$ and $\sigma_{v_x} = \sigma_{v_y} = 5m/s$. To account for measurement noise, we use the values $\sigma_{R} = 0.035m$, $\sigma_{\Omega} = \pi/4$, and $\sigma_{V} = 0.1807m/s$, which are the range, spatial frequency, and Doppler bin sizes, respectively. In the absence of an exact ground truth of the target's position and velocity per frame, track-level fusion estimates\cite{4648063} provide a reasonable benchmark for comparison with our one-shot estimates. For each configuration (A-C), while evaluating the performance of one-shot fusion for each trajectory (straight/random), we utilize the calibration results obtained using the other trajectory to ensure fairness.

Firstly, we compare the performance of Bayesian and ML approaches for one-shot fusion in Table~\ref{tab:oneshot}, focusing on root mean square error (RMSE) values, which indicate the difference between instantaneous and track-level fused position/velocity estimates. While ML approaches often perform comparably to Bayesian methods, they struggle with uncertainties arising from trajectories and radar configurations. In setup B1, depicted in Fig. {\color{blue} Add B1 uncertainty figure}, the target's velocity vector is perpendicular to the position vectors from the two radars, leading to uncertainty because neither radar can provide radial Doppler information. Whereas, in configuration C, where the radars face each other, shown in Fig. {\color{blue} Add configuration C uncertainty figure}, both radars can only measure one velocity component, causing uncertainty. Without prior knowledge of the distributions of $v_x$ and $v_y$, the ML approach yields unreliable estimates, especially in these high-uncertainty scenarios.

The RMSE values in Table~\ref{tab:oneshot} show significantly worse performance for ML in Configuration C compared to B1, as the high uncertainty in B1 affects only a short segment of the trajectory, whereas Configuration C experiences this uncertainty consistently. Thus, the Bayesian approach proves more robust in noisy and uncertain environments for one-shot fusion.

Using Table~\ref{tab:oneshot}, we can compare the performance of Bayesian one-shot fusion across the different configurations. We observe that configuration B yields the best position RMSE values among the three setups, while configurations A and C deliver comparable results. Additionally, among all the random trajectory setups (A2, B2, C2), setup B2 achieves the best velocity RMSE value. Configuration B1 performs worse than B2 due to the trajectory-based uncertainty previously discussed. In conclusion, configuration B demonstrates the best overall one-shot fusion performance among all the setups presented, as it offers the maximum field of view (FoV) diversity. Conversely, configuration C ranks the lowest due to having the least FoV diversity, as both radars in this configuration face each other.

Finally, in Fig. \ref{fig:one_shot_fusion}, we present a qualitative comparison of the position estimates $(X, Y)$ and velocity estimates $(V_X, V_Y)$ obtained through four different methods: 1) the Extended Kalman Filter (EKF) at \(R_1\), 2) the EKF at \(R_2\) transformed to the frame of reference of \(R_1\), 3) track-level fusion, and 4) one-shot fusion, specifically for configuration B2. We observe that the EKF estimates from \(R_1\) and \(R_2\) closely align, indicating a qualitative validation of the self-calibration approach. Although the one-shot estimates for velocities (\(V_X, V_Y\)) are generally less accurate than those from track-level fusion and the individual EKF estimates, one-shot fusion has a notable advantage: it can generate estimates using measurements from just a single frame.

To fully realize the potential of the Bayesian approach, we estimate the state covariance matrix using the posterior distribution. This provides a measure of the uncertainties associated with the state estimates. For instance, in Fig.~\ref{fig:uncertainty}, we illustrate the uncertainties in velocity across two regions by using the velocity posterior distribution. This method allows us to obtain one-shot estimates of both the state and the state covariance, which can be beneficial in low-latency scenarios.


%For the Bayesian one-shot fusion, we consider suitable iid Gaussian priors (\ref{Prior Distributions}). Since velocity estimates have higher uncertainty than position, we consider $\sigma_x, \sigma_y=1$ and $\sigma_{v_x}, \sigma_{v_y}=5$. Additionally, we select $\sigma_{R}=0.035$, $\sigma_{\Omega}=\pi/4$, and $\sigma_{V_R}=0.36$ for modeling the measurement noise.

\begin{comment}
In the absence of an exact ground truth of the target's position and velocity per frame, track-level fusion estimates {\color{blue} (reference for the track level fusion?)} provide a reasonable benchmark for comparison. In Fig.~\ref{fig:one_shot_fusion} we have provided a qualitative comparison of the position $(X, Y)$ and velocity $(V_X, V_Y)$ estimates obtained by 1) the EKF at $R_1$, 2) the EKF at $R_2$, transformed to $R_1$'s frame of reference, 3) track-level fusion and 3) one-shot fusion, for the configuration B2. However, for a quantitative performance evaluation of the one-shot fusion, we illustrate the RMSE values in Table~\ref{tab:oneshot} (the difference between the instantaneous and track-level fused position/velocity estimates). We notice that in most of the setups, the performance of ML-based one-shot fusion is comparable to its Bayesian counterpart. However, in B1, the ML approach has a worse performance because it yields unstable estimates in high uncertainty scenarios (Fig.~\ref{fig:uncertainty}). Additionally, the ML estimate is significantly worse in configuration C, where the other radar is at the broadside of the reference. As shown in the diagram ({\color{blue}Point to picture}), both radars are only able to measure the radial component ($v_x$) of the target at each frame, and have no information about $v_y$. Therefore, without knowledge about the prior distribution of $v_y$, the ML approach will lead to unreliable estimates, which will impact instantaneous velocity estimation. Therefore, the Bayesian approach yields robust one-shot estimates in noisy and high-uncertainty scenarios. 
\end{comment}

\begin{table}[t!]
  \centering
  \renewcommand{\arraystretch}{1.3}

  % Wrap tabular in \resizebox
  \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}l S S c S S c S S@{}}
      \toprule
      & \multicolumn{2}{c}{$A$} & \phantom{abc}& \multicolumn{2}{c}{$B$} &
        \phantom{abc} & \multicolumn{2}{c}{$C$} \\
      \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(lr){8-9}
      & {$1$} & {$2$} && {$1$} & {$2$} && {$1$} & {$2$}\\
      \midrule
      \multicolumn{1}{l}{\textbf{Position RMSE}}\\
      Bayesian & 0.3333 & 0.3287 && 0.1708 & 0.1439 && 0.3748 & 0.3694 \\
      ML       & 0.3404 & 0.3248 && 0.1701 & 0.1438 && 0.3839 & 0.3691 \\
      \multicolumn{1}{l}{\textbf{Velocity RMSE}}\\
      Bayesian & 0.3634 & 0.3233 && 0.3448 & 0.2668 && 0.7671 & 0.8135 \\
      ML       & 0.3639 & 0.3239 && 0.3439 & 0.2667 && {\bfseries 9.7155} & {\bfseries 6.0543} \\
      \bottomrule
    \end{tabular}
  }%

  \caption{RMSE for one-shot fusion (Bayesian vs ML). Values indicated in bold indicate cases when ML estimates fail}
  \label{tab:oneshot}
\end{table}

==> preliminary.tex <==
\section{Measurement Model}

\begin{figure}[t!] % Use figure* for spanning both columns
 \centering 
 %\vspace{-0.4cm}
\includegraphics[scale = 0.6]{measurementmodel.png} 
\caption{Measurement model for a single moving target seen by a radar with respect to a global frame of reference}
\label{fig:measurementmodel}
\vspace{-0.6cm}
\end{figure}

We first introduce the basic measurement model for a radar $Radar_i$ tracking a single moving target described in Fig.~\ref{fig:measurementmodel}. Although we evaluate our approach on humans (extended targets), we have considered a point-target model for this abstraction. So, while evaluating the performance on the actual data, we will consider the detection-cluster centroids as point targets, which can be used to denote the motion of the entire human body. Let positions of $Radar_i$ and the target w.r.t. a global frame of reference be $(x_i, y_i)$ and $(x, y)$ respectively, while the target velocity is given by $(v_x, v_y)$. The orientation of $Radar_i$ w.r.t the global frame is $\phi_i$. Let us denote them with vectors $\mathbf{p_i}=(x_i, y_i)^T$, $\mathbf{p}=(x, y)^T$ and $\mathbf{\dot{p}}=(v_x, v_y)^T$. We want to get expressions for the estimated measurements of the target by $R_i$. 

The range estimate $r_i$ is given by:

\EQ \label{range_estimate}
    r_{i} = \| \mathbf{p} - \mathbf{p_i} \| = \sqrt{(x - x_{i})^{2} + (y - y_{i})^{2}}
\EN

The radial Doppler $v_i$ is obtained by taking the projection of the target velocity vector
v onto the unit vector that points from the radar to the target:

\EQ \label{Doppler_estimate}
    v_{i} = \langle {\mathbf{\dot{p}}, \frac{\mathbf{p}-\mathbf{p_i}}{\| \mathbf{p} - \mathbf{p_i} \|}} \rangle
    = \frac{v_{x}\,(x - x_{i}) + v_{y}\,(y - y_{i})}{r_{i}}
\EN

where $\langle {\mathbf{a},\mathbf{b}} \rangle = \mathbf{a}^T \mathbf{b}$ is the inner product of vectors $\mathbf{a}$ and $\mathbf{b}$.

\noindent Let $\mathbf{\hat{\mu_i}}=(\cos{\phi_i}, \sin{\phi_i})^T$ denote the unit vector along the radar array length. Then the spatial frequency of the target w.r.t $Radar_i$ is given as $\omega_{i} = \pi\sin{\theta}$ where $\theta$ is the angle subtended by the target on $Radar_i$. This can be calculated as follows:

\EQ \label{spatial_frequency_estimate}
\omega_{i} = \frac{\pi\langle {\mathbf{p} - \mathbf{p_i}, \mathbf{\hat{\mu_i}}} \rangle}{r_i}
=\frac{((x-x_i)\cos{\phi_i}+(y-y_i)\sin{\phi_i})}{r_i}
\EN
